Inclusive Design of AI's Explanations: Just for Those Previously Left Out, or for Everyone?

Motivations: Explainable Artificial Intelligence (XAI) systems aim to improve users' understanding of AI, but XAI research shows many cases of different explanations serving some users well and being unhelpful to others. In non-AI systems, some software practitioners have used inclusive design approaches and sometimes their improvements turned out to be "curb-cut" improvements -- not only addressing the needs of underserved users, but also making the products better for everyone. So, if AI practitioners used inclusive design approaches, they too might create curb-cut improvements, i.e., better explanations for everyone. Objectives: To find out, we investigated the curb-cut effects of inclusivity-driven fixes on users' mental models of AI when using an XAI prototype. The prototype and fixes came from an AI team who had adopted an inclusive design approach (GenderMag) to improve their XAI prototype. Methods: We ran a between-subject study with 69 participants with no AI background. 34 participants used the original version of the XAI prototype and 35 used the version with the inclusivity fixes. We compared the two groups' mental model concepts scores, prediction accuracy, and inclusivity. Results: We found four main results. First, it revealed several curb-cut effects of the inclusivity fixes: overall increased engagement with explanations and better mental model concepts scores, which revealed fixes with curb-cut properties. However (second), the inclusivity fixes did not improve participants' prediction accuracy scores -- instead, it appears to have harmed them. This "curb-fence" effect (opposite of the curb-cut effect) revealed the AI explanations' double-edged impact. Third, the AI team's inclusivity fixes brought significant improvements for users whose problem-solving styles had previously been underserved. Further (fourth), the AI team's fixes reduced the gender gap by 45%.

==> Content/Future_Work.tex <==
\section{Future Work **DELETE ME**} 
% **MMH: D2**
% \boldification{Our next step is to check gendermag survey responses. The results showed that GenderMag fixes improved mental model. Now we want to examine participants' problem solving styles and the usability issues they faced during the study.}

\NOTE{MMB: I'm not a fan of "future work" sections in journal papers. They're not interesting, and we already did part of them.  Bottom line: cut this section.}

In this ongoing research, our next step involves analyzing the GenderMag survey responses that we gathered from both groups of participants. Findings from the previous section suggested the positive impact of GenderMag fixes on user experiences that led to better mental model concepts scores for the Post-GenderMag participants. Now, we plan to closely examine participants' problem-solving styles. In the GenderMag survey, participants responded what are their problem-solving styles in different scenarios. We plan to analyze their reported problem-solving styles and the usability issues they mentioned during the user study.

\par 
% \boldification{we want to know what happened to Abi- and Tim-like when they used the Pre-GM and the Post-GM versions}
During the GenderMag-driven cognitive walkthroughs, Team Game adopted the Abi persona, recognizing the support needed for Abi-like users' problem-solving styles. Our aim is to investigate whether the Original and the Post-GenderMag versions posed challenges for Abi-like users, what specific issues they encountered, and the differences between the two versions in terms of the usability issues. Subsequently, we want to check if Team Game's GenderMag fixes worked for our Abi-like Post-GenderMag participants. Finally, we aim to know that Team Game's GenderMag fixes did not inadvertently cause any usability issues for users with Tim's problem-solving styles.


==> Content/GlobalTODOs.tex <==
\begin{itemize}
    \item VOCAB: Fixing the "Fix" names: throughout the paper, appendix, figures the fix names should be consistent. [Done] % double check, fix table in methods/results/appendix
    
    \item VOCAB: Code is a concept now. [Done]
    
    \item VOCAB: no 'mentioned' with participants' quote replace with a more active sounding verb, some suggestions: pointed out, called out, wrote about, remarked, put it [Done]
    
    \item VOCAB: special fixes replace with 'most referred to' [Done] % double check "special" language isn't there 
    
    \item VOCAB: special concept replace with differentiating concept [Done]
    
    \item VOCAB: AgentSense replace with How Agent Behaves [Done]

    \item GRAMMAR:  "criterion" is singular, "criteria" is plural (ie,  more than one criterion).  [Done]

    \item MISC: Add Puja in the author list [Done]
    \item Author: Add Jon? (Montaser will ask Dr. B) [Done]
    
    \item FIGURES: In figures, have separate patterns for Tim and Abi so that readers can easily distinguish. [Done]


% 6. We changed the prediction loss a bit: we used max(negative score, 0) to reward participants who predicted square with higher score than the square that the agent took, but the overall picture was the same: the results can be found here: https://docs.google.com/spreadsheets/d/1kkAlJSoTZMy5gT6d0sK4AWln8QO8GE7tFx-WsshQ_pg/edit#gid=621711220

    \item WRITING: Prediction loss results new story: The after participants were faithful to historical data for predicting the next best move for the agent, but it did not cut it. Following the gameboard was better. [Done]

    \item TODO: Discussion Question: Be careful what you wish for out of your explns. goes to results and again in the discussion. [Done]

    \item AUDIT: Softmax is not part of the discussion story anymore. [Done]

    \item carriage return fix with Twiddle \~ : before referencing figures and tables, also before cite [Done]

    \item Fix-10 in Table fix-examples: do we need to keep this as we don't have engagement with explanation as a separate section? [Done]
    
    \item WRITING: avoid describing Team Game's "inside-the-heads" states (eg, avoid "believed", "felt", ...) -- replace with actions (but do be sure you KNOW they happened from what they said/wrote), eg: "decided", "concluded", "said", "wrote", ... [Done]
    
    \item problem-solving style or facet? [Done] % outside GM section use style

    \item make the facet name's first letter uppercase for each word [Done] **MMB: needs a recheck: I think I broke this rule in the Results sections about Fix-2 and Fix-7, maybe elsewhere too?
    FAM: I re-checked 11/27 11:48 am**
    
    \item Use more descriptive phrase for the three explanations- BTW, STT, OTB
BestToWorst, ScoresThroughTime, OnTheBoard [Done] % also add changes in methodology

    \item No more Team J, it's Team Game now. [Done]

    \item STATS: DF is lower case df [Done] % FAM: Degrees of freedom do not appear in paper except for hidden comments / tables

    \item Change inclusivity support to just inclusivity [Done]
    
    \item When reporting results/stats Post-GM should come before Original [Done]
    
    \item Use one word for participant 'response'/comment/feedback/writings/statements/written comments/remarks [Done] % we analyzed participant's responses ( use when referring to participant data, not referencing what they said)
    
    \item Anything with data should start with people. [Done]

    \item checking all the figure, table, footnote references and their captions, footnote text; if figure references to a part of the figure use "Figure #: Position" [Done] % stopped after methodology
    
    \item Mental Model scores should be replaced by Mental Model Concepts scores [Done] % FAM: checked once, round back to section 3.4 measuring mental models to see if it still makes sense
    
% FAM: Final checks
    \item Check all footnotes. Their positions, link. [Done **check positions once boldifs/notes are cleared]

    \item use "PredError" instead of "Prediction Performance", Use PredError in place of prediction loss **there is some inconsistency between PredError(s), PredError scores, PredError rates...** [Done]  % when talking generally say prediction accuracy

    \item Important: "Prediction Performance" is not a THING, it's just a way to SCORE Mental Models.  Never talk about it like a thing (never use the term), and never contrast it as a thing with Mental Models. Use Prediction Accuracy when talking in general [Done] % FAM: I am confused on what this means for the RQs in the introduction as readers will not know what prediction loss scores mean

    \item Really really Important: Mental Models are a THING, and the ONLY Thing in this paper.  Never contrast it with Prediction Performance (which is NOT a thing).  When we talk about good/better Mental MOdels, we're talking abstractly.  When we're talking about SCORES, those are:\\
    "Mental Model Concepts Scores" not "Mental Models" and \\
    "Prediction Loss Scores" not "Prediction Performance".. [Done, 11/25 11:45am]

    \item Global search and replace highlight with suggest or something similar [Done]

    \item Add acknowledgment [Done]
    
    \item Check for section name capitalization  consistency, particularly subsections [Done]

    \item Remove unused figures/assets in figures folder [Done] 

    \item Check if shortened version "PredErr" is still around [Done]

    \item Say #-tailed t test not SIDE in results [Done]

\end{itemize}


==> Content/LEFTOVERS-relatedwork.tex <==
% // Guidelines for XAI and measuring mental models
\boldification{Many guidelines and processes exist for developing and evaluating XAI--but **few** address diverse problem-solving styles.}
As mentioned in the previous paragraphs, numerous guidelines and processes exists for developing and evaluating XAI systems but few address users' diverse problem-solving styles.
Works like Amershi et al. proposed and tested a set of 18 guidelines for human-AI interactions that span across different points of interactions with an AI product~\cite{Amershi19Guide}.
Hoffman et al.~\cite{hoffman2023measures} proposed several measures that evaluate the quality, user satisfaction, and user understanding of the explanations. 
In our study, we used a form of Hoffman et al.'s prediction tasks, glitch (flaw) detection task, and task reflection to deduce participant's mental models.
We also used some items from the explanation satisfaction scale for participant feedback.
These works focus on the features and quality of the AI and its interactions, however, it does not account for how different users may approach the system.


% THIS IS THE OLD OLD VERSION

\boldification{recent HAI works focus on a lot things but we are interested in cognitive diversity}
In recent years, Human-AI Interaction (HAI) research has focused on user performance, system reliability, trustworthiness, and safety~\cite{shneiderman20human}, while also exploring the dynamics of human and AI control levels~\cite{shneiderman22human}. The growing body of HAI works aims to increase transparency~\cite{Rader06Tr}, explain AI behaviors~\cite{Herlocker00Exp, Kulesza15Principles}, provide guidelines for AI practitioners~\cite{Amershi19Guide}, and address ethical principles in governance~\cite{Shneiderman21RAI}. Additionally, HAI research advocates for human-centric concerns such as well-being, privacy, and cognitive capacities in the adoption of AI technologies~\cite{ozmen2023six, shneiderman22human}. In our study, we are specifically interested in bringing diverse users' problem-solving styles together with HAI to improve XAI's inclusivity.

\subsection{Problem-Solving Style and HAI/XAI **D??**}

\boldification{Here are some examples of works that investigate participants' cognitive styles}
There's been limited investigation into how users' problem-solving styles influence HAI/XAI. Although AI researchers have examined users' explanation preferences, they've largely overlooked individual differences within these preferences~\cite{Dodge19Fairness}. Some research used users' cognitive diversity to understand why users behave or judge differently when interacting with AI systems.
% The definitions of cognitive styles vary as different works may measure cognitive styles differently. HAI research commonly defines cognitive styles as the “need for cognition”. XAI and HAI researchers widely used this definition, often to gather participants' data in such a way that they can analyze results based on their need for cognition. 
For example, when looking at how fair end-users' perception of AI was, Dodge et al.~\cite{Dodge19Fairness} assessed the impacts of two factors: i) four types of explanations and ii) data processing. Their findings revealed that participants' need for cognition significantly impacted their perception of the AI's fairness. Similarly, Millecamp et al.'s work~\cite{Millecamp20Cognitive} found that diverse end-users' cognitive styles showed differences in their trends to interact with the AI's explanations. This investigation discussed that the variation in the definitions of cognitive styles did not have much effect and any of the definition variations could help identify valuable insights.
\par

\boldification{There are other definitons of cognitive styles that have been used to evaluate human-AI interaction.}
Goldberg et al.~\cite{Goldberg90AnA} presented an alternative approach to capturing individual differences through five personality traits--- Openness, Conscientiousness, Extraversion, Agreeableness, and Neuroticism (OCEAN)~\cite{Goldberg90AnA}. They found that one of the personality traits, ``Openness'' influenced users' interaction with the interface. Jiang et al.~\cite{Jiang00Expert} also used a personality trait, self-confidence to evaluate participants' acceptance of the expert system's output. Other researchers also used some form of problem-solving styles, cognitive styles, and personality traits to explain user behavior~\cite{Giboney12Acceptance, Kulesza12Mental, felmingham21importance, djulbegovic14evaluation}. However, none of these works considered a wider range of problem-solving styles as we did in our study.
\par

\boldification{In this paper we use the five GenderMag facets to define cognitive styles}
In this study, we used problem-solving styles defined by users'--- attitude towards risk, computer self-efficacy, motivations, information processing style, and learning style.

\subsection{GenderMag **D??**} 
\label{sec:methodology_gendermag}

\boldification{GenderMag is a usability inspection method}
We used the GenderMag method to define the end users' five problem-solving style ranges used in this study. GenderMag, also known as the Gender-Inclusiveness Magnifier, is a usability inspection method to find and fix gender-inclusivity bugs in problem-solving software~\cite{Hamid23GM, Burnett16GM, Guizani22Inlcusivity, Vorvoreanu19Bias}. This method focuses on five facets of gender differences (statistical), brings them to life through three faceted personas, and encapsulates the use of these facets into a systematic process through a gender specialization of the Cognitive Walkthrough (CW)~\cite{Wharton94CW}. Software practitioners have used this method to evaluate the software they design and develop from a gender-inclusiveness perspective~\cite{Burnett16GM, Guizani22Inlcusivity, Vorvoreanu19Bias}.

\par
\boldification{GenderMag defines 5 facets or problem-solving styles}
The GenderMag method’s five facets capture five factors in an individual’s problem-solving style: their motivations for using technology, information processing styles, computer self-efficacy, attitude toward risk in using unfamiliar technology features, and learning style (by process vs. by tinkering)~\cite{Burnett16GM, Hamid23GM}. The ``inclusivity bugs'' uncovered by GenderMag are instances where a technology product fails to fully accommodate the complete range of values associated with the five facets, leading to a disproportionate impact on individuals whose problem-solving styles are unsupported. These bugs are also considered gender-inclusivity issues because the facets reflect statistical differences among gender preferences in problem-solving styles~\cite{Burnett16GM, Guizani22Inlcusivity, Vorvoreanu19Bias, Hamid23GM}. GenderMag reveals inclusivity issues that are statistically associated with gender preferences. GenderMag does not use peoples' gender identities to find inclusivity concerns, it uses only their problem-solving styles.

\par
\boldification{GenderMag brings these facets to life with 3 research based personas}
The GenderMag method has three personas: Abi (Abigail/Abishek), Pat (Patricia/Patrick), and Tim (Timara/Timothy) (see Table \ref{tab:facets}). Statistically, the problem-solving styles of Abi disproportionately skew toward women, for Tim they disproportionately skew toward men, and Pat provides a third set of values within Abi and Tim~\cite{Burnett16GM, Hamid23GM}.

\begin{table}[h]
    \centering
     \caption{Three GenderMag personas and their problem-solving styles.}
    \label{tab:facets}
    \begin{tabular}{p{3cm}|p{3cm}|p{3cm}|p{3cm}}
     & \multicolumn{1}{c|}{\includegraphics[width=1.8cm, height=1.8cm]{figures/Abi.png}} &\multicolumn{1}{c|}{\includegraphics[width=1.8cm, height=1.8cm]{figures/Pat.png}}  & \multicolumn{1}{c}{\includegraphics[width=1.8cm, height=1.8cm]{figures/Tim.png}}\\ & \textbf{Abigail/Abishek ("Abi")} & \textbf{Patricia/Patrick ("Pat")} & \textbf{Timara/Timothy ("Tim")} \\
    \hline
    Attitude Toward Risk &  Risk-Averse & Risk-Averse & Risk-Tolerant \\
    \hline
    Self-Efficacy &  Lower & Medium & Higher \\
    \hline
    Motivations &  Task-Oriented & Task-Oriented & Tech-Oriented \\
    \hline
    Information Processing Style &  Comprehensive & Comprehensive & Selective \\
    \hline
    Learning: by Process vs. by Tinkering &  Process-Oriented & Learns by tinkering: tinkers reflectively & Learns by tinkering (sometimes to excess) \\
    \hline
    \multicolumn{4}{l}{\footnotesize Abi and Tim have problem-solving styles at each facet's endpoints, and Pat has a mix of possible facet values.}
    \end{tabular}
\end{table}
\par

\boldification{GenderMag weaves the facets and personas together through a specialized form of cognitive walkthrough}
The GenderMag faceted personas are integrated into a systematic specialized Cognitive Walkthrough process. A group of evaluators adopt a specific GenderMag persona, say Abi, customize the persona’s background (optional), and systematically ``walkthrough'' each step of a use case. At each step, they answer three questions: i) will <Abi> have formed this subgoal as a step to their overall goal? why?, ii) will <Abi> take the action the developers expected at this step? Why?, and iii)  if <Abi> took the action, will they know that they did the right thing and are making progress toward their goal? Why? If the evaluators find any answer is negative because of Abi's particular problem-solving styles, they report an inclusivity bug, provide their reasons, and note down the problem-solving styles that support their reasonings. Later, when fixing an inclusivity bug, these notes ensure that the fixes are designed around Abi's problem-solving styles that highlighted the bug.

\par

\boldification{In this study, the evaluators were AI practitioners}
The evaluators relevant to our study were a group of AI practitioners whom we called ``Team Game'' in this paper. Team Game evaluated their own XAI prototype from the perspective of the Abi persona. They chose the Abi persona as Abi represents the group of users who are most often left out of the development process which results in more barriers for these users. Team Game's before GenderMag and after GenderMag version of the prototype were then used in our study.


\subsection{XAI in Sequential Domains}

\boldification{What is sequential domain}
The AI practitioners of our study designed their XAI prototype specifically for a sequential domain. A sequential domain refers to a specific situation or area where actions or events unfold in a particular order, following a series of steps or stages in a predetermined sequence. For instance, consider a board game like Chess, where players take turns making moves and the progression of the game follows an ordered sequence of moves. In recent years, there has been a growing interest in developing AI systems that can play sequential games like Chess, Shogi, and Go. This has led to the development of AI players that can compete with and even outperform the world champions of these games~\cite{Silver16Go, Silver18RL}. Real-Time Strategy (RTS) games have also seen similar achievements~\cite{Vinyals19GM, Vinyals19alphastar}. 

\par

\boldification{explaining AI players' actions in sequential domains is challenging}
 Despite such progress, explaining AI players' actions in sequential domains remains a major challenge. In an attempt to understand this challenge, Metoyer et al.~\cite{Metoyer10RTS} studied how experienced users explain strategies and gameplay in RTS games. In another study, Penney et al.~\cite{Penney18Foraging} found that even experienced users encounter challenges when seeking information about an intelligent agent in an RTS setting. One result was that participants showed a preference for ``What'' information over ``Why''. In a sequential game domain, understanding the causal relationships among relevant variables within the game can also help users~\cite{Madumal20Explain}. As Madumal et al.~\cite{Madumal20Explain} showed offering causal explanations of AI agents can enhance participants' ability to predict tasks, as well as increase their satisfaction and trust. In another study, Dodge et al.~\cite{Dodge22Rank} observed that when ranking AI agents playing a sequential game like Tic-Tac-Toe, participants highlighted the importance of detailed explanations to differentiate between closely matched agents. That study also noted that participants showed a preference for receiving multiple explanations over a single one when making decisions.   


\subsection{Mental Models and Explainable AI (XAI)}
\boldification{AI systems are hard to understand}
The opaque nature of AI systems poses a challenge for end-users with low or no expertise in AI~\cite{Wortham17Robot, Tsai22Logic}. This especially hinders users' ability to seamlessly interpret and trust the system's output~\cite{Kulesza15Principles}. Lim et. al~\cite{Lim09Context} regarded such lack of clarity as an intelligibility concern for AI systems. 


\boldification{explanations can improve the mental model of users}
To improve the clarity of an AI system, researchers and developers often provide explanations of the system to its end-users~\cite{Alipour21Improving, Brachman23Following, Schraagen20Trusting, Pierson23Comparing}. According to Hoffman et al., explanations that are effective and satisfactory for users can facilitate the development of a good mental model~\cite{hoffman2019metrics}. Kulesza et al. demonstrated that providing explanations about the debugging process of a machine-learning system improved participants' understanding of the system~\cite{Kulesza15Principles, Kulesza10Debug}. Also, the explanations improved their participants' ability to rectify errors. Other studies also found additional benefits of adding explanations such as improvements in users' self-reported satisfaction~\cite{Kapoor10Interactive, Amershi14Power} and feelings of trust towards the AI systems~\cite{Lim09Context, Tsai21Exploring, Schraagen20Trusting}. 

\par

\boldification{Measuring Mental models in XAI}
Mental models have been captured using different methods including questionnaires about the agent, mental model drawings, and task performance~\cite{Brachman23Following, Schraagen20Trusting, Zhang24Fair, Bansal19Beyond, Alipour21Improving}. 
Hoffman et al.~\cite{hoffman2019metrics} proposed measures that evaluate the quality, user satisfaction, and user understanding of the explanations. According to Hoffman et al., mental models can be deduced from empirical evidence, even though individuals might find it challenging to fully articulate their understanding~\cite{hoffman2019metrics}. However, the authors suggested that through guided task reflection, people can effectively communicate their understanding of an event or system, including its fundamental concepts and principles. The authors provided a list of 11 methods that researchers have used to derive mental models across various domains, including cognitive psychology, expert system knowledge acquisition, instructional design, and educational computing. From these 11 methods, Anderson et al. used the ``Prediction Task'' and ``Task Reflection'' to understand users' mental models of a Reinforcement Learning agent~\cite{Anderson19RL}. In our paper, we have utilized these two methods and also integrated the ``Glitch Detector Task'',  and ``Self-Explanation Task'' from Hoffman et al.'s 11 methods to know if users were able to find any flaws in the given explanations and their own understanding of the AI agent. 

\par

\boldification{Our work is different}
Thus, although HAI and XAI research have made significant progress in exploring users' mental models, they often overlooked the potential impact of users' diverse problem-solving styles on their overall understanding of AI systems. Recognizing this gap, we wanted to check the effectiveness of GenderMag-driven cognitive walkthroughs that put users' diverse problem-solving styles at the center stage of finding and fixing inclusivity issues.  
Historically, HCI practitioners leveraged GenderMag for a wide variety of user experience improvements such as inclusivity bug removal~\cite{Guizani22Inlcusivity}, task performance improvement~\cite{Vorvoreanu19Bias}, customer rating improvement~\cite{Burnett17MS}, etc. However, no prior GenderMag research has evaluated GenderMag's applicability and effectiveness within AI-powered systems. Addressing this gap in GenderMag studies, our goal is to investigate how successful GenderMag fixes can be in improving users' engagement and their mental models of AI.




% --------------------------------------------------------------------------------------------------------------
\boldification{As AI becomes more common, XAI literature has sought to improve AI products to address challenges in trust, decision making, task performance, error correction, safety, transparency control, understanding, and satisfaction.}
\NOTE{trust in the decisions of AI , user's understanding of AI, task performance ? do we mention the meaning/definition?}
As AI becomes more common, many XAI works sought to address challenges in AI adoption and usage such as trust, understanding, and task performance.
Trusting AI output, especially when it involves potential harm to the user, is an important measure to consider.
\NOTE{For the below line , add a sentence on why }
Tsai et al.~\cite{Tsai21Exploring} examined transparency and explainability in an online symptom checker and found that explanations improved users' trust, understanding, and satisfaction with the diagnosis compared to the baseline. 
To address the challenge of making AI decisions more transparent, Zhang and Lim (2022) developed the XAI Perceptual Processing Framework which is designed to provide more relatable and cognitively aligned explanations for AI decisions, particularly in vocal emotion recognition.
Their framework incorporates different types of explanations like contrastive saliency, counterfactual examples, and contrastive cues to help users better interpret the decisions of AI.
Their findings revealed that counterfactual samples improved decision-making and trust by allowing users to explore "what-if" scenarios, making AI decisions more transparent and understandable~\cite{Zhang22Relatable}.

% FM: below fits with human aspect
In a similar branch, Danry et al.~\cite{Danry23Tell} proposed AI framed questions, that is explanations that are framed as questions rather than simply providing feedback, to improve co-reasoning interaction between AI systems and humans. The participants were tasked with validating the logical validity of the statements related to socially divisive topics by considering the logic themselves rather than passively accepting the AI’s reasoning, by shifting participants from passive receivers to active evaluators of logic. This method led to increase in discernment accuracy of flawed statements as compared to other conditions like no explanations or Causal AI explanations.


\boldification{User factors (cognitive styles, problem solving styles, need for cognition, biases) impact how they interact with the AI system and therefore worth investigating how XAI can be better designed to meet those needs.}

% Several examples of XAI techniques include counterfactual, example, and feature explanations all of which enhance users' understanding of AI decisions~\cite{Alipour21Improving, Tsai21Exploring, Dodge19Fairness}.
% Improving users' mental models of AI systems by designing error boundaries that are parsimonious and non-stochastic, making it easier for humans to understand when the AI is likely to err~\cite{bansal2019beyond}.
% Dodge's fairness paper connects to mental models via: you must have some understanding/perception on how AI reached its decision in order to evaluate fairness

% below makes less sense here and also not really true
% Works in XAI often target the expert user though there are works demonstrating the need to address the lay user~\cite{ehsan24who, tsai22logic}. 





% current
\boldification{Our work is different as it examines how inclusivity methods, namely GenderMag, can improve mental models of AI. GenderMag has been used in a variety of non-AI works.}
% **A lot of work has been studying different explanations' effect on users, but few cater to the users' needs. Our work differs by offering a A/B test for using inclusive design methods to inform design changes to XAI systems with the goal of improving users' mental models of the system and thus their experience.**
Recognizing this gap, we investigated the effectiveness of GenderMag as an inclusive design approach to improve users' mental models of AI systems by putting users’ diverse problem-solving styles at the center stage of finding and fixing inclusivity issues.
% Within the XAI space, HCI researchers have used GenderMag to measure the inclusivity of AI products.
Historically, HCI practitioners have leveraged GenderMag for a wide variety of user experience improvements such as inclusivity bug removal~\cite{Guizani22Inlcusivity}, automated inclusivity bug detection in online courseware~\cite{Chatterjee22Inclusivity}, task performance improvement~\cite{Vorvoreanu19Bias}, customer rating improvement~\cite{Burnett17MS},  etc. 
Researchers also used GenderMag within AI contexts such as measuring AI products' inclusivity ~\cite{anderson2024measuring} and examining software developers' use of generative AI~\cite{Choudhuri24Guides}.
However, previous GenderMag studies have not examined GenderMag's potential to improve users' mental models of AI systems.
To address this gap, we investigated how successfully GenderMag-driven inclusivity fixes could improve users' mental models of AI in a formal experimental setting.

% two pargraphs to lead in with inclusive design:
% past works of GM, inclusivity in AI work gap -> how we are difference
% don't have to add / cite new works for 2nd part

% None of these works attempted to use x, hence we're filling this gap. 


%FAM: v2
\boldification{Our work is different as it examines how inclusivity methods, namely GenderMag, can improve mental models of AI. GenderMag has been used in a variety of non-AI works.}
% **A lot of work has been studying different explanations' effect on users, but few cater to the users' needs. Our work differs by offering a A/B test for using inclusive design methods to inform design changes to XAI systems with the goal of improving users' mental models of the system and thus their experience.**
Recognizing this gap, we investigated the effectiveness of GenderMag as an inclusive design approach to improve users' mental models of AI systems by putting users’ diverse problem-solving styles at the center stage of finding and fixing inclusivity issues.
Historically, HCI practitioners have leveraged GenderMag for a wide variety of user experience improvements such as inclusivity bug removal~\cite{Guizani22Inlcusivity}, automated inclusivity bug detection in online courseware~\cite{Chatterjee22Inclusivity}, task performance improvement~\cite{Vorvoreanu19Bias}, customer rating improvement~\cite{Burnett17MS},  etc. 
Researchers also used GenderMag within AI contexts such as measuring AI products' inclusivity ~\cite{anderson2024measuring} and examining software developers' use of generative AI~\cite{Choudhuri24Guides}.
% However, previous GenderMag studies have not examined GenderMag's potential to improve users' mental models of AI systems.
However, previous GenderMag studies have not examined inclusive design's potential to improve users' mental models of AI systems.

% \boldification{
% GenderMag has a track record of improving software for users through inclusive design approaches. 
% Many works sought to improve users' mental models through XAI techniques and considering human factors, inclusive design is the next step. 
% Inclusivity design methods offer a holistic way to target users }
\boldification{Our work differs by examining what inclusive design methods can offer for targeting XAI problems---explanations, interface, and human factor.}
Our work examines what inclusive design methods can offer for tackling XAI design concerns---encompassing the explanations, system, and the human in the interaction.
Inclusive design methods, namely GenderMag, focuses on users' diverse problem-solving styles to generate actionable design directions. 
% Thus, inclusive design methods offer a way to consider both design concerns in XAI, techniques and the human factor.
To address this gap, we investigated how successful inclusive design methods, specifically GenderMag, could improve users' mental models of AI in a formal experimental setting.
% To address this gap, we investigated how successfully GenderMag-driven inclusivity fixes could improve users' mental models of AI in a formal experimental setting.



% FAM: v3
\boldification{Our work differs by examining what inclusive design methods can offer for addressing design concerns in XAI---techniques and the human factor.}
Recognizing this gap, we investigated the effectiveness of GenderMag as an inclusive design approach to improve users' mental models of AI systems by putting users’ diverse problem-solving styles at the center stage of finding and fixing inclusivity issues.
Historically, HCI practitioners have leveraged GenderMag for a wide variety of user experience improvements such as inclusivity bug removal~\cite{Guizani22Inlcusivity}, automated inclusivity bug detection in online courseware~\cite{Chatterjee22Inclusivity}, task performance improvement~\cite{Vorvoreanu19Bias}, customer rating improvement~\cite{Burnett17MS},  etc. 
Researchers also used GenderMag within AI contexts such as measuring AI products' inclusivity ~\cite{anderson2024measuring} and examining software developers' use of generative AI~\cite{Choudhuri24Guides}.
% However, previous GenderMag studies have not examined GenderMag's potential to improve users' mental models of AI systems.
However, previous GenderMag studies have not examined inclusive design's potential to improve users' mental models of AI systems.
Our work differs by examining what inclusive design methods can offer for addressing design concerns in XAI---both the techniques and the human factor.
**Inclusive design methods like GenderMag focus on users' diverse problem-solving styles to generate actionable design directions.**
To address this gap, we investigated how successfully GenderMag-driven inclusivity fixes could improve users' mental models of AI in a formal experimental setting.



==> Content/OldRelatedWork.tex <==
\section{Related Works and Background}
\subsection{User Characteristics and HAI/XAI. **D1?}
\boldification{The extent to which researchers consider and leverage user characteristics in XAI/HAI.}
There is a vast number of empirical works where HAI researchers work towards investigating end-users’ interactions with AI-based products and systems. Yet, these works often lack either (1) gathering sufficient data on the characteristics and the cognitive styles of the products’ end-users or (2) they collect the data, but do not factor in the data in their work.

\boldification{Examples of researchers not gathering or gathering but not considering users' characteristics/ cognitive styles}
Exemplifying (1), Poursabzi-Sangdeh et al. investigated how users interacted with an AI product that predicted apartment prices. They had 3,800 participants but did not collect participants’ demographic data which could have played a role in the explanatory factor~\cite{Poursabzi21Manipulating}. An example for (2) is when Lee et al.~\cite{Lee20GUICOMP} investigated participants' feelings while using a system. This work found that GUIComp was perceived as beneficial and effective by participants. This investigation collected participants’ gender and age. However, Lee et al. did not use participants’ data on gender or age to measure the differences in the level of comfort participants felt with the GUIComp.

\boldification{Here are some works that include participants' characteristics}
Within the works that do include participants' characteristics, demographics, and behavioral diversity, there are some interesting findings. For example, Pal et al.\cite{Pal2019UserEW} accounted for participants' English proficiency. More specifically, they measured the level of satisfaction participants had while using voice assistants, leading to results which showed that native English speaker's level of satisfaction was higher than those of non-native speakers. Other works such as Derrick \& Ligon et al.~\cite{Derrick14Affect} and Graaf et al.~\cite{Graaf15Sharing} found that there were outside factors like participants’ gender differences when evaluating how willing participants were to accept robotic technologies and how likeable they thought an AI was, respectively. In addition to gender, Graaf et al. also looked at the age factor when participants evaluated the AI. When looking at other characteristics such as race and ethnicity, Kim et al.\cite{Kim23One} found that minority group participants within these characteristics show a more positive attitude and sense of goodwill towards AI. Similarly, compared to female participants, male participants showed a better attitude towards AI. Other works also studied end-users’ cultural background~\cite{Shahid14Child}, people’s trust in government~\cite{Chen20Self}, sex~\cite{Lee00Computer}, and people’s experience with computer vision~\cite{Bansal19Accuracy}. These works investigated how the listed characteristics influenced the perception of AI systems. However, limitations exist such as not having enough data from 
particular demographic groups (e.g., non-white participants)~\cite{Harrison20Empirical}. This can prevent HAI researchers from further investigating how factors such as participants’ characteristics and cognitive styles unfairly affect end-users’ interactions with AI products. 

\boldification{Here are some examples of works that investigate participants' cognitive styles}
Few investigations have dug into finding how cognitive styles can play a role in human-AI interaction. Within this area of research, the definitions of cognitive styles vary as different works may measure cognitive styles differently. One such definition that is used in human-AI interaction research is “need for cognition”. XAI and HAI researchers widely used this definition, often to gather participants' data in such a way that they can analyze results based on their need for cognition. For example, when looking at how fair end-users' perception of AI was, Dodge et al.~\cite{Dodge19Fairness} used two factors. These included four types of explanations and the influence of data processing. Their findings showed that participants' need for cognition revealed significant differences in their perception of the AI's fairness. Similarly, Millecamp et al.'s work~\cite{Millecamp20Cognitive} found that diverse end-users' cognitive styles showed differences in their trends to interact with the AI's explanations. This investigation discussed that the variation in the definitions of cognitive styles do not have much effect, and that valuable insights can be identified using any of the definition variations.

\boldification{There are other definitons of cognitive styles that have been used to evaluate human-AI interaction.}
One variation of the definition for cognitive styles presented by Goldberg~\cite{Goldberg90AnA} is capturing participants cognitive styles through five traits. This is their Openness, Conscientiousness, Extraversion, Agreeableness, and Neuroticism (OCEAN). When studying end-users' use of the AI music recommendation system Millercamp et al.~\cite{Milecamp20User} used this definition. Other definitions are based on the tendency of end-users to form stereotypes~\cite{Giboney12Acceptance}.

\boldification{In this paper we use the five GenderMag facets  to define cognitive styles}
In this work, we define cognitive styles as end-users' problem-solving styles shaped by their attitude towards risk, computer self-efficacy, motivations, information processing style, and learning style (by process vs. by tinkering).

\subsection{GenderMag}

\boldification{GenderMag is a usability inspection method to find and fix gender-inclusiveness bugs in technology}
The five porblem-solving styles we mentioned above came from GenderMag. GenderMag, also known as the Gender-Inclusiveness Magnifier, is a usability inspection method to find and fix gender-inclusivity bugs in problem-solving software. This method can be used by software practitioners to evaluate the software they design and develop from a gender-inclusiveness perspective.  GenderMag method focuses on five facets of gender differences, brings them to life through three faceted personas and encapsulates use of these facets into a systematic process through a gender specialization of the Cognitive Walkthrough (CW) [citeme: ].

\boldification{GenderMag defines 5 facets or cognitive styles}
The GenderMag method’s five facets of captures an individual’s cognitive style, which guides their interaction with capture an individual's diversity of motivations for using technology, their information processing styles, their computer self-efficacy, their attitude toward risk in using unfamiliar technology features and their learning style (by process vs. by tinkering) [1]. The "inclusivity bugs" uncovered by GenderMag are instances where a technology product fails to fully accommodate the complete range of values associated with the five facets, leading to a disproportionate impact on individuals whose cognitive styles are unsupported. These bugs are also considered gender-inclusivity issues because the facets reflect statistical differences among gender preferences in cognitive styles [citeme:]. 

\boldification{GenderMag brings these facets to life with 3 research based personas}
The GenderMag method introduces three personas, namely Abi (Abigail/Abishek), Pat (Patricia/Patrick), and Tim (Timara/Timothy). The facet values represented by the Abi persona are disproportionately skew towards women, the facet values represented by Tim are disproportionately skew towards men, and Pat provides a third set of values within Abi and Tim [citeme:]. A portion of Abi and Tim persona are shown in Figure X and Figure Y. [add personas here]

\boldification{GenderMag weaves the facets and personas together through a specialized form of cognitive walkthrough}
The GenderMag faceted personas are integrated into a systematic specialized Cognitive Walkthrough (CW) process. During this evaluation, the evaluators adopt a specific GenderMag persona (say Abi), customize the persona’s background (optional) and systematically “walkthrough” each step of a use case. They then respond to questions related to the persona's sub-goals and actions for completing the use case. For instance, Will <Abi > have formed this subgoal as a step to their overall goal? (Yes/no/maybe, why, and the facets attached). If the evaluators find Abi would not have formed the subgoal because of their underlying facet, then there is an inclusivity bug. By following this process, evaluators can find inclusivity bugs in their UI along with their corresponding facets, which are crucial to the fixes. Inclusivity bugs can be addressed effectively by designing fixes around the specific facets that highlighted the inclusivity bugs.

\boldification{something to close this and make a continuation for next: Need to talk with Montaser}


\subsubsection{}

\subsection{Human-Centered evaluation of AI}
\subsubsection{Metrics used for Human-centric evaluation of AI}

\boldification{Human-centered evaluation metrics}

HAI Researchers use human-centered evaluation metrics to obtain valuable insights into end-user performance during interactions with AI systems, as well as the systems' impact on them. These metrics help in understanding how transparent, trustworthy, fair, accountable, and explainable AI systems are. They are also vital for making sure AI follows ethical and legal rules and for dealing with any biases or unintended consequences. Mohseni et al., [161] categorize human-centered evaluation metrics into four groups:  human-AI task performance, mental model, user trust, and the usefulness and satisfaction of explanations. In this subsection, we will discuss these metrics as well as a few others that are commonly used for the human-centric evaluation of AI. 

\boldification{Human-AI Task performance}
Human-AI task performance refers to how effectively and efficiently a person engages with or employs an artificial intelligence system to complete a particular task. The usual way to assess human-AI task performance is by measuring the percentage of correctly predicted instances in the decision-making process~\cite{Yao22HCAI, Kunel19Let, Raha20Causal, Ingrid20System}. Other popular human-AI task performance evaluation metrics include task completion times, error rates, user satisfaction surveys, and cognitive load~\cite{Bertucci23Dendromap, Aly17Metric}. Along with task performance, user engagement metrics are often used to measure the extent of user involvement and interest during interactions with AI systems~\cite{Ghazarian20Predictive}. These metrics, such as interaction duration, click-through rates, and task completion rates, eye movement serve as proxies for determining the level of user engagement while performing tasks using AI systems~\cite{Sabrina15Recognition, Bertucci23Dendromap}.

\boldification{Trust and user satisfaction help evaluate the user acceptance of AI systems}
Trust and user satisfaction are two crucial measurement metrics in evaluating user acceptance of AI systems. Stanton er al.,\cite{Stanton21NIST} mentioned that when evaluating the trustworthiness, we need to consider factors such as accuracy, reliability, and explainability, along with various system characteristics of the AI technologies. Additionally, trust evaluation often includes self-reported trust measurement from users as leveraged by Ajenaghughrure et al.,\cite{Ajenaghughrure21Psycho}. The most commonly used method for measuring user trust is through surveys, followed by interviews and focus groups~\cite{Bach22System}. The other user acceptance evaluation metric, user satisfaction refers to the level of fulfillment a user experiences when using an AI system. One commonly used method for assessing user satisfaction is through the use of post-interaction surveys, where users provide ratings on a Likert scale to indicate their level of satisfaction~\cite{hoffman2019metrics}. For example, Brooke proposed the System Usability Scale (SUS) that provides a standardized assessment of usability~\cite{Brooke95SUS}. Questionnaires like the Explanation Satisfaction Scale are also used to assess user satisfaction with AI system's explanations~\cite{hoffman2019metrics}. Van der Waa et al.,\cite{Jasper21XAI} and Bilgic et al.,~\cite{Bilgic05Explain} also showed that interviews can offer a comprehensive understanding of user satisfaction .


\boldification{Fairness, Interpretability}
When it comes to promoting transparency and mitigating biases in an AI system, interpretability and fairness emerge as the two pivotal evaluation metrics. Hardt et al.,\cite{Moritz16Equality} highlight that fairness is crucial to avoid discriminatory results that can eventually create disadvantaged groups in AI systems. Evaluating fairness through metrics such as disparate impact analysis, demographic parity, and equal opportunity allows for the measurement and reduction of biases in the algorithmic decision-making processes of the systems~\cite{Moritz16Equality, Floridi20Social}. Interpretability is another vital characteristic of an AI system that enhances transparency and ensures that the system's workflows, outcomes, and explanations, are easily understandable to users. Some common measures of interpretability include post-hoc explanation methods like LIME (Local Interpretable Model-agnostic Explanations)~\cite{Tulio16Trust} and quantitative metrics such as feature importance scores\cite{Srinivasu22Blackbox, Janet21Roadmap}.



\boldification{Users' mental model} 
In HAI, Measuring users' mental model refers to the measurement of user understanding of an AI system~\cite{anderson2020mental}. This understanding can be categorized as global, local, and functional understanding~\cite{Janet21Roadmap}. At a basic level, researchers evaluate users' understanding by evaluating their understanding of the accuracy of an AI system. This can be done by assessing users' understanding of the system's current states and functions~\cite{Epley2007OnSH, Rutjes19Consider}. At a more advanced level, researchers assess users' ability to predict future states and reduce uncertainty during interactions with the AI system~\cite{Epley2007OnSH, Rutjes19Consider}. To assess whether users have understood an AI system is typically done through tasks that require the users to recollect and reflect on their mental models of concepts~\cite{Baumberger17Explain, hoffman2019metrics}. Subjective measures like questionnaires are also used to evaluate user comprehension~\cite{hoffman2019metrics}. Additionally, in educational contexts, participants often take tests that check their objective understanding of the AI system at various stages of the learning process~\cite{Zheng19Video}.


\subsubsection{Methods for Human-centric evaluation of AI}

\boldification{Human-Centric evaluation of AI systems}
HAI researchers emphasize the evaluation of AI systems, recognizing the need for user-centric design to facilitate effective collaboration between humans and AI. They use a variety of methods to evaluate AI systems from an end-user standpoint. 

\boldification{Interviews and Observations}
One commonly used method is interviews and observations. Interviews serve as a means to collect user experiences and perceptions of the AI system, while observations offer insights into how users engage with the system in practical, real-world scenarios. Beede et al. demonstrated the application of interviews and field observations in characterizing end-user experiences with an AI-powered system~\cite{Beede20Clinic}. Their observational data provide insights into what healthcare professionals anticipate and the difficulties they face when incorporating AI-assisted technology into their workflows.
End-user Interviews are also popular in understanding users' AI literacy\cite{Kaspersen21teaching, Watkins20Literacy, Ng21Literacy}. However, it is important to note that interviews and observations may have limitations. For instance, the sample size may be too small to minimize bias and individual subjectivity and it takes a long time to code the data~\cite{Ng21Literacy, Tang20Assess}. 

\boldification{Surveys}
A potential way to address the limitation of interviews and observation is by conducting surveys. With surveys, it's comparatively easier to gather valuable insights and feedback from a large number of users. For example, Zander et al. conducted a survey among 377 patients and 80 medical professionals, to investigate their knowledge, experience, and opinion of AI in healthcare\cite{Zander22health}. Conducting interviews or observing these many participants would have been an extremely difficult task and would require tremendous effort and resources. Despite the advantages, surveys or questionnaire studies are also subject to a few limitations. First, users may respond to surveys based on their preconceived notions or personal preferences, which may not always align with the actual performance or effectiveness of the AI system\cite{Jeff16Survey}. Second, user surveys rely on self-reported data, which may not always accurately reflect users' true experiences or behaviors\cite{Latkin16Survey}. 

\boldification{Usability Testing}        
Usability testing, as an alternative, offers a more interactive and engaging approach to involve participants in a user study. This method is particularly effective in collecting real-time usage data, pinpointing usability issues, and obtaining both qualitative and quantitative feedback on AI systems. For instance, Anderson et al. conducted a controlled lab study with 124 participants to explore variations in users' mental models of a reinforcement learning agent based on different types of visual explanations~\cite{Anderson19RL}. In another controlled lab study, Dodge et al., recruited 10 participants to gain insights into how people rank multiple AI agents when observing them in action~\cite{Dodge22Rank}.  In studies like these, where participants' active interaction with AI systems is crucial, usability testing emerges as the more fitting approach.

\boldification{There are other methods also}
In addition to the methods outlined above, researchers employ various other approaches to assess AI systems from an end-user perspective. These include A/B testing\cite{Bertucci2022DendroMap}, task performance metrics\cite{Gunning_Aha_2019}, longitudinal studies\cite{Fidas23Longitudinal}, and more. Each of these methods offers unique insights into the user experience, contributing to a comprehensive evaluation of the AI system's effectiveness and user-friendliness.

\boldification{Which methods we have used in our study}
To get a clearer understanding of our participant's mental models, we wanted to create an interactive experience for them. That's why we conducted usability testing with two groups of participants in a Between-Subject study. The ``Before'' group participants used the ``Before'' version of the interface and the ``After'' group participants used the ``After'' version. To provide more structure to the assessment process we used AAR/AI(After Action Review for AI)\cite{Theresa20AAR, Dodge21AAR, Dodge22Rank}. AAR/AI helped our participants to focus on assessment perspectives such as identifying what happened and examining why it happened. It's worth noting that, AAR/AI was also used with XAI interfaces before. Khanna et al. demonstrated that participants who utilized AAR/AI identified more bugs compared to those who did not utilize this methodology\cite{Khanna22AAR}. In section 3 we discussed the AAR/AI questions and the other details of our study design.     

% \boldification{we should evaluate user mental models too}
% Furthermore, the design of AI systems should consider the views and mental models of the users. To capture and evaluate the interactions between users and AI systems, researchers have incorporated insights from cognitive and perceptual psychology, as well as social sciences. By including theoretical principles from these disciplines, researchers can account for human preconceptions about the inner workings and behavior of AI systems. This not only helps explain users' expectations, fears, and trust issues towards AI systems but also allows researchers to design AI systems that align with human understanding and needs.


% End users evaluate AI systems in user studies through various methods and criteria, taking into account factors such as accuracy, usefulness, transparency, usability, and their overall experience with the technology.  Firstly, when considering accuracy, users evaluate the alignment of AI system predictions with their expectations and assess if the information provided is reliable, helping them make well-informed decisions [**refaccuracy**]. For example, Alharbi et al. found that users are more likely to trust the accuracy of an app if they have a good understanding of how the app works and if they believe that the app is aligned with their expectations. 




 

% \boldification{Frameworks and Guidelines for Human-Oriented Assessment of AI}
% When it comes to measuring technology adoption and acceptance among users, there exist numerous frameworks and guidelines that follow a more human-centered approach. Technology Acceptance Model(TAM) is an example of such a framework. TAM helps in predicting how much a group of users will like a system and why some people or smaller groups might feel differently about it. Another popular technology acceptance model, the Unified Theory of Acceptance and Use of Technology(UTAUT) integrates both TAM and the Theory of Reasoned Action (TRA) to explain usage behavior and user intention. More specifically, this model uses four core determinants for predicting user behavior: 1) performance expectancy, 2) effort expectancy, 3) social influence, and 4) facilitating conditions. In the HAI domain, we can use models like TAM and UTAUT for measuring the acceptance of an AI system but they do not provide any assessment process for AI [**CIte Jon's Paper**]. Moreover, there is no existing research on how different problem-solving styles of end users can be associated with the key constructs of acceptance models like TAM and UTAUT.  


% \boldification{AAR/AI}

\subsection{Mental Models and XAI}

\boldification{AI systems are hard to understand}
To understand an AI system better, it's important to explore the system's underlying methods and workflows used for data handling and decision-making. This can potentially help users form a robust mental model of how the AI system works. However, the inherent opaque nature of AI poses a significant challenge for end-users with low or no expertise in the field\cite{Wortham17Robot}. This especially hinders users' ability to seamlessly interpret and fully trust the system's outputs\cite{Kulesza15Principles}. Lim et. al~\cite{Lim09Context}, regarded such lack of clarity as an intelligibility concern for AI systems. 

\boldification{explanations can improve the mental model of users}
To improve the clarity of an AI system, Researchers and developers often provide explanations of the system to the end-users. According to Hoffman et al., explanations that are effective and satisfactory for users can facilitate the development of a good mental model\cite{hoffman2019metrics}. Kulesza et al. demonstrated that providing explanations about the debugging process of a machine-learning system improved participants' understanding of the system~\cite{Kulesza15Principles, Kulesza10Debug}. Also, the explanations enhanced participants' ability to rectify errors. Other studies also found additional benefits of adding explanations to an AI system. This includes improvements in users' self-reported satisfaction~\cite{Kapoor10Interactive, Amershi14Power} and feelings of trust towards the AI systems\cite{Lim09Context}. 

\boldification{Measuring Mental models in XAI}
Hoffman et al.~\cite{hoffman2019metrics} address the question of explaining AI systems to users and propose measures that gauge the quality of explanations, user satisfaction with the explanations, user comprehension of the explanations, and factors such as user trust and reliance on AI systems. According to Hoffman et al., mental models can be deduced from empirical evidence, even though individuals might find it challenging to fully articulate their understanding\cite{hoffman2019metrics}. However, the authors suggest that through guided task reflection, people can effectively communicate their understanding of an event or system, including its fundamental concepts and principles. The authors provided a list of eleven methods that researchers have used to derive mental models across various domains, including cognitive psychology, expert system knowledge acquisition, instructional design, and educational computing. From these 11 methods, Anderson et al. used the ``Prediction Task'' and ``Task Reflection'' to understand users' mental models of a Reinforcement Learning agent\cite{Anderson19RL}. In our paper, we have utilized those two methods and also added the ``Glitch Detector Task'',  and ``Self-Explanation Task'' to know whether users are able to find any flaws in the given explanations and their own understanding of the AI agent. Differing from the study conducted by Anderson et al., our participants submitted their confidence scores for the prediction task. Also, we analyzed user responses both qualitatively and quantitatively whereas Anderson et al. relied on qualitative analysis only.     

\boldification{Our work is different}
While most works on explanation and mental models provide a more realistic user-centric assessment of AI systems, they do not delve into the potential influence of users' distinct problem-solving styles on their individualized understanding of AI. This particular shortcoming of XAI research inspired us to focus on users' cognitive styles and how we can utilize user differences to fix inclusivity bugs of an XAI interface.

% Furthermore, beyond the information presented by the AI system, users' domain expertise also acts as a critical factor in evaluating the effectiveness of an AI system~\cite{Kim18Performance}[**need more citation**]. 






\subsection{XAI in Sequential Domains}

\boldification{What is sequential domain}
A sequential domain refers to a specific situation or area where actions or events unfold in a particular order, proceeding one after the other. It can be compared to following a series of steps or stages in a predetermined sequence. For instance, consider a board game like Chess, where players take turns making moves and the progression of the game follows an ordered sequence of moves. In recent years, there has been a growing interest in developing AI systems that can play sequential games like Chess, Shogi, and Go. This led to the development of AI players that can not only compete with but also outperform the world champions of those games~\cite{Silver16Go, Silver18RL}. similar achievements were also made with Real-Time Strategy (RTS) games~\cite{Vinyals19GM, Vinyals19alphastar}. 

\boldification{explaining AI players' actions in sequential domains is challenging}
 Despite such progress, explaining AI players' actions in sequential domains remains a major challenge. In an attempt to understand this challenge, Metoyer et al.~\cite{Metoyer10RTS} studied how experienced users explain strategies and gameplay in RTS games. In another study, Penney et al.\cite{Penney18Foraging} found that even experienced users encounter challenges when seeking information about an intelligent agent in an RTS setting.  When it comes to explanations, the authors noted that participants showed a preference for ``What'' information over ``Why''. In a sequential game domain, understanding the causal relationships among relevant variables within the game can also help users. As shown by Madumal et al.~\cite{Madumal20Explain}, offering causal explanations of AI agents can enhance participants' ability to predict tasks, as well as increase their satisfaction and trust. In another study, Dodge et al.~\cite{Dodge22Rank} observed that when ranking AI agents engaged in a sequential game like Tic-Tac-Toe, participants highlighted the importance of detailed explanations to differentiate between closely matched agents. The researchers also noted that participants showed a preference for receiving multiple explanations over a single one when making decisions. 

   


\subsection{Agent and Explanation}
% refer to https://dl.acm.org/doi/pdf/10.1145/3490099.3511115 [Section 3]
\boldification{The Agent is built with a CNN and is tasked with predicting outcome tuple O = Win, Loss, Draw.}

The agent~\cite{Dodge22Rank} playing the MNK game and generating explanations has a Convolutional Neural Network is tasked with predicting outcome tuples $O = (Win\%, Loss\%, Draw\%)$ for each square on the $M \times N$ board. 
The network has an input layer with 2 channels for each agent's pieces on the board. 
The input tensors goes through 5 convolutional layers, 2 fully connected layers, and ending with a sigmoid layer for the final output. 
The ReLU activation function is used throughout. The output shape is $(M \times N \times O)$, where $O$ is the set of outcomes.
\boldification{**FM**: Is the generalization value function GVF the same thing as the Agent calculating the score Win-Loss? From my understanding the GVF is how an agent assesses/evaluates how good an action is. (p.s. I forgot how to leave general comments)}
The agent selects actions by using a forward pass on the network to get the predicted outcomes and then applying a generalized value function~\cite{Sutton11Horde}. 
For each square, the agent scores it by using the function $Win\% - Loss\%$ and then applies a Gumbel-Softmax function to the scores. 
The agent then samples the resulting distribution to pick a near-max value action.  
In the backward pass, the authors~\cite{Dodge22Rank} computed L1Loss between the network's output and target values; and computed proportions for win, loss, and draw from the results of the game rollouts which become regression targets.

\boldification{Explanation 1: BTW}
The agent has three explanations in the interface where it presents the scores of each square. 
In the Best to Worst (BTW)  explanation presents each score of the 36 squares on the board as a rectangle with the best score on the left to the worst on the right.
Illegal decisions are assigned very low scores.
After each move by the agent the participant is predicting, a new series of rectangles will appear in the explanation and the prior set of scores is in a lighter color. 
The most recent series will be the darkest color.
\boldification{**FM**: Maybe put Before behavior and then cover changes in Methodology to reduce confusion.}
Before: hovering over a square on the gameboard will highlight the score of that square in all decision points.
After: hovering over a square on the gameboard will highlight its corresponding score in the explanation.
Also hovering over a score in the explanation will reveal a tooltip that present the (Win\%, Loss\%, Draw\%)
In both versions of the prototype, only the most recent series has interactive highlighting. 

\boldification{Explanation 2: STT}
The Scores Through-Time (STT) presents a time component to the agent where it shows how the agent scored each score at each decision. 
The X-axis is time and when the agent makes a decision a new column of scores appears.
The score with the maximum score in the column is highlighted in a darker color for the current move. 
Hovering over a gameboard square will highlight its score for every decision through time.
Hovering over a score in the column highlights its corresponding square in the gameboard and the score of that square in prior decisions.
A new column is generated after the game progresses one step.

\boldification{Explanation 3: OTB}
The last explanation, Scores On-the-Board (OTB), presents a relation of time and space by representing each square's score over time in its own chart. 
So this explanation contains 36 charts that match the same format as STT.
Hovering over a square in the gameboard highlights the corresponding chart in the explanation and vice versa.
A new data point is added to each chart after the agent takes an action.


==> Content/Vocab.tex <==
**Vocab stuff moved to GlobalTODOs


==> Content/commands.tex <==
\FIXME
\boldification
\colorbox{mylimegreen} for Original participants (only in figure and captions)
\colorbox{mysteelblue} for Post-GM participants (only in figure and captions)




==> Content/v1RelatedWork.tex <==
\section{Related Works and Background}
% // Guidelines for XAI and measuring mental models
% \boldification{Many guidelines and processes exist for developing and evaluating XAI--but **few** address diverse problem-solving styles.}
% As mentioned in the previous paragraphs, numerous guidelines and processes exists for developing and evaluating XAI systems but few address users' diverse problem-solving styles.
% Works like Amershi et al. proposed and tested a set of 18 guidelines for human-AI interactions that span across different points of interactions with an AI product~\cite{Amershi19Guide}.
% Hoffman et al.~\cite{hoffman2023measures} proposed several measures that evaluate the quality, user satisfaction, and user understanding of the explanations. 
% In our study, we used a form of Hoffman et al.'s prediction tasks, glitch (flaw) detection task, and task reflection to deduce participant's mental models.
% We also used some items from the explanation satisfaction scale for participant feedback.
% These works focus on the features and quality of the AI and its interactions, however, it does not account for how different users may approach the system.


% THIS IS THE OLD OLD VERSION

\boldification{recent HAI works focus on a lot things but we are interested in cognitive diversity}
In recent years, Human-AI Interaction (HAI) research has focused on user performance, system reliability, trustworthiness, and safety~\cite{shneiderman20human}, while also exploring the dynamics of human and AI control levels~\cite{shneiderman22human}. The growing body of HAI works aims to increase transparency~\cite{Rader06Tr}, explain AI behaviors~\cite{Herlocker00Exp, Kulesza15Principles}, provide guidelines for AI practitioners~\cite{Amershi19Guide}, and address ethical principles in governance~\cite{Shneiderman21RAI}. Additionally, HAI research advocates for human-centric concerns such as well-being, privacy, and cognitive capacities in the adoption of AI technologies~\cite{ozmen2023six, shneiderman22human}. In our study, we are specifically interested in bringing diverse users' problem-solving styles together with HAI to improve XAI's inclusivity.

\subsection{Problem-Solving Style and HAI/XAI }

\boldification{Here are some examples of works that investigate participants' cognitive styles}
There's been limited investigation into how users' problem-solving styles influence HAI/XAI. Although AI researchers have examined users' explanation preferences, they've largely overlooked individual differences within these preferences~\cite{Dodge19Fairness}. Some research used users' cognitive diversity to understand why users behave or judge differently when interacting with AI systems.
% The definitions of cognitive styles vary as different works may measure cognitive styles differently. HAI research commonly defines cognitive styles as the “need for cognition”. XAI and HAI researchers widely used this definition, often to gather participants' data in such a way that they can analyze results based on their need for cognition. 
For example, when looking at how fair end-users' perception of AI was, Dodge et al.~\cite{Dodge19Fairness} assessed the impacts of two factors: i) four types of explanations and ii) data processing. Their findings revealed that participants' need for cognition significantly impacted their perception of the AI's fairness. Similarly, Millecamp et al.'s work~\cite{Millecamp20Cognitive} found that diverse end-users' cognitive styles showed differences in their trends to interact with the AI's explanations. This investigation discussed that the variation in the definitions of cognitive styles did not have much effect and any of the definition variations could help identify valuable insights.
\par

\boldification{There are other definitons of cognitive styles that have been used to evaluate human-AI interaction.}
Goldberg et al.~\cite{Goldberg90AnA} presented an alternative approach to capturing individual differences through five personality traits--- Openness, Conscientiousness, Extraversion, Agreeableness, and Neuroticism (OCEAN)~\cite{Goldberg90AnA}. They found that one of the personality traits, ``Openness'' influenced users' interaction with the interface. Jiang et al.~\cite{Jiang00Expert} also used a personality trait, self-confidence to evaluate participants' acceptance of the expert system's output. Other researchers also used some form of problem-solving styles, cognitive styles, and personality traits to explain user behavior~\cite{Giboney12Acceptance, Kulesza12Mental, felmingham21importance, djulbegovic14evaluation}. However, none of these works considered a wider range of problem-solving styles as we did in our study.
\par

\boldification{In this paper we use the five GenderMag facets to define cognitive styles}
In this study, we used problem-solving styles defined by users'--- attitude towards risk, computer self-efficacy, motivations, information processing style, and learning style.

\subsection{GenderMag} 
\label{sec:methodology_gendermag}

\boldification{GenderMag is a usability inspection method}
We used the GenderMag method to define the end users' five problem-solving style ranges used in this study. GenderMag, also known as the Gender-Inclusiveness Magnifier, is a usability inspection method to find and fix gender-inclusivity bugs in problem-solving software~\cite{Hamid23GM, Burnett16GM, Guizani22Inlcusivity, Vorvoreanu19Bias}. This method focuses on five facets of gender differences (statistical), brings them to life through three faceted personas, and encapsulates the use of these facets into a systematic process through a gender specialization of the Cognitive Walkthrough (CW)~\cite{Wharton94CW}. Software practitioners have used this method to evaluate the software they design and develop from a gender-inclusiveness perspective~\cite{Burnett16GM, Guizani22Inlcusivity, Vorvoreanu19Bias}.

\par
\boldification{GenderMag defines 5 facets or problem-solving styles}
The GenderMag method’s five facets capture five factors in an individual’s problem-solving style: their motivations for using technology, information processing styles, computer self-efficacy, attitude toward risk in using unfamiliar technology features, and learning style (by process vs. by tinkering)~\cite{Burnett16GM, Hamid23GM}. The ``inclusivity bugs'' uncovered by GenderMag are instances where a technology product fails to fully accommodate the complete range of values associated with the five facets, leading to a disproportionate impact on individuals whose problem-solving styles are unsupported. These bugs are also considered gender-inclusivity issues because the facets reflect statistical differences among gender preferences in problem-solving styles~\cite{Burnett16GM, Guizani22Inlcusivity, Vorvoreanu19Bias, Hamid23GM}. GenderMag reveals inclusivity issues that are statistically associated with gender preferences. GenderMag does not use peoples' gender identities to find inclusivity concerns, it uses only their problem-solving styles.

\par
\boldification{GenderMag brings these facets to life with 3 research based personas}
The GenderMag method has three personas: Abi (Abigail/Abishek), Pat (Patricia/Patrick), and Tim (Timara/Timothy) (see Table~\ref{tab:facets}). Statistically, the problem-solving styles of Abi disproportionately skew toward women, for Tim they disproportionately skew toward men, and Pat provides a third set of values within Abi and Tim~\cite{Burnett16GM, Hamid23GM}.

\begin{table}[h]
    \centering
     \caption{Three GenderMag personas and their problem-solving styles}
    \label{tab:facets}
    \begin{tabular}{p{3cm}|p{3cm}|p{3cm}|p{3cm}}
     & \multicolumn{1}{c|}{\includegraphics[width=1.8cm, height=1.8cm]{figures/Abi.png}} &\multicolumn{1}{c|}{\includegraphics[width=1.8cm, height=1.8cm]{figures/Pat.png}}  & \multicolumn{1}{c}{\includegraphics[width=1.8cm, height=1.8cm]{figures/Tim.png}}\\ & \textbf{Abigail/Abishek ("Abi")} & \textbf{Patricia/Patrick ("Pat")} & \textbf{Timara/Timothy ("Tim")} \\
    \hline
    Attitude Toward Risk &  Risk-Averse & Risk-Averse & Risk-Tolerant \\
    \hline
    Self-Efficacy &  Lower & Medium & Higher \\
    \hline
    Motivations &  Task-Oriented & Task-Oriented & Tech-Oriented \\
    \hline
    Information Processing Style &  Comprehensive & Comprehensive & Selective \\
    \hline
    Learning: by Process vs. by Tinkering &  Process-Oriented & Learns by tinkering: tinkers reflectively & Learns by tinkering (sometimes to excess) \\
    \hline
    \multicolumn{4}{l}{\footnotesize Abi and Tim have problem-solving styles at each facet's endpoints, and Pat has a mix of possible facet values.}
    \end{tabular}
\end{table}
\par

\boldification{GenderMag weaves the facets and personas together through a specialized form of cognitive walkthrough}
The GenderMag faceted personas are integrated into a systematic specialized Cognitive Walkthrough process. A group of evaluators adopt a specific GenderMag persona, say Abi, customize the persona’s background (optional), and systematically ``walkthrough'' each step of a use case. At each step, they answer three questions: i) will <Abi> have formed this subgoal as a step to their overall goal? why?, ii) will <Abi> take the action the developers expected at this step? Why?, and iii)  if <Abi> took the action, will they know that they did the right thing and are making progress toward their goal? Why? If the evaluators find any answer is negative because of Abi's particular problem-solving styles, they report an inclusivity bug, provide their reasons, and note down the problem-solving styles that support their reasonings. Later, when fixing an inclusivity bug, these notes ensure that the fixes are designed around Abi's problem-solving styles that highlighted the bug.

\par

\boldification{In this study, the evaluators were AI practitioners}
The evaluators relevant to our study were a group of AI practitioners whom we called ``Team Game'' in this paper. Team Game evaluated their own XAI prototype from the perspective of the Abi persona. They chose the Abi persona as Abi represents the group of users who are most often left out of the development process which results in more barriers for these users. Team Game's before GenderMag and after GenderMag version of the prototype were then used in our study.


\subsection{XAI in Sequential Domains}

\boldification{What is sequential domain}
The AI practitioners of our study designed their XAI prototype specifically for a sequential domain. A sequential domain refers to a specific situation or area where actions or events unfold in a particular order, following a series of steps or stages in a predetermined sequence. For instance, consider a board game like Chess, where players take turns making moves and the progression of the game follows an ordered sequence of moves. In recent years, there has been a growing interest in developing AI systems that can play sequential games like Chess, Shogi, and Go. This has led to the development of AI players that can compete with and even outperform the world champions of these games~\cite{Silver16Go, Silver18RL}. Real-Time Strategy (RTS) games have also seen similar achievements~\cite{Vinyals19GM, Vinyals19alphastar}. 

\par

\boldification{explaining AI players' actions in sequential domains is challenging}
 Despite such progress, explaining AI players' actions in sequential domains remains a major challenge. In an attempt to understand this challenge, Metoyer et al.~\cite{Metoyer10RTS} studied how experienced users explain strategies and gameplay in RTS games. In another study, Penney et al.~\cite{Penney18Foraging} found that even experienced users encounter challenges when seeking information about an intelligent agent in an RTS setting. One result was that participants showed a preference for ``What'' information over ``Why''. In a sequential game domain, understanding the causal relationships among relevant variables within the game can also help users~\cite{Madumal20Explain}. As Madumal et al.~\cite{Madumal20Explain} showed offering causal explanations of AI agents can enhance participants' ability to predict tasks, as well as increase their satisfaction and trust. In another study, Dodge et al.~\cite{Dodge22Rank} observed that when ranking AI agents playing a sequential game like Tic-Tac-Toe, participants highlighted the importance of detailed explanations to differentiate between closely matched agents. That study also noted that participants showed a preference for receiving multiple explanations over a single one when making decisions.   


\subsection{Mental Models and Explainable AI (XAI)}
\boldification{AI systems are hard to understand}
The opaque nature of AI systems poses a challenge for end-users with low or no expertise in AI~\cite{Wortham17Robot, Tsai22Logic}. This especially hinders users' ability to seamlessly interpret and trust the system's output~\cite{Kulesza15Principles}. Lim et. al~\cite{Lim09Context} regarded such lack of clarity as an intelligibility concern for AI systems. 


\boldification{explanations can improve the mental model of users}
To improve the clarity of an AI system, researchers and developers often provide explanations of the system to its end-users~\cite{Alipour21Improving, Brachman23Following, Schraagen20Trusting, Pierson23Comparing}. According to Hoffman et al., explanations that are effective and satisfactory for users can facilitate the development of a good mental model~\cite{hoffman2019metrics}. Kulesza et al. demonstrated that providing explanations about the debugging process of a machine-learning system improved participants' understanding of the system~\cite{Kulesza15Principles, Kulesza10Debug}. Also, the explanations improved their participants' ability to rectify errors. Other studies also found additional benefits of adding explanations such as improvements in users' self-reported satisfaction~\cite{Kapoor10Interactive, Amershi14Power} and feelings of trust towards the AI systems~\cite{Lim09Context, Tsai21Exploring, Schraagen20Trusting}. 

\par

\boldification{Measuring Mental models in XAI}
Mental models have been captured using different methods including questionnaires about the agent, mental model drawings, and task performance~\cite{Brachman23Following, Schraagen20Trusting, Zhang24Fair, Bansal19Beyond, Alipour21Improving}. 
Hoffman et al.~\cite{hoffman2019metrics} proposed measures that evaluate the quality, user satisfaction, and user understanding of the explanations. According to Hoffman et al., mental models can be deduced from empirical evidence, even though individuals might find it challenging to fully articulate their understanding~\cite{hoffman2019metrics}. However, the authors suggested that through guided task reflection, people can effectively communicate their understanding of an event or system, including its fundamental concepts and principles. The authors provided a list of 11 methods that researchers have used to derive mental models across various domains, including cognitive psychology, expert system knowledge acquisition, instructional design, and educational computing. From these 11 methods, Anderson et al. used the ``Prediction Task'' and ``Task Reflection'' to understand users' mental models of a Reinforcement Learning agent~\cite{Anderson19RL}. In our paper, we have utilized these two methods and also integrated the ``Glitch Detector Task'',  and ``Self-Explanation Task'' from Hoffman et al.'s 11 methods to know if users were able to find any flaws in the given explanations and their own understanding of the AI agent. 

\par

\boldification{Our work is different}
Thus, although HAI and XAI research have made significant progress in exploring users' mental models, they often overlooked the potential impact of users' diverse problem-solving styles on their overall understanding of AI systems. Recognizing this gap, we wanted to check the effectiveness of GenderMag-driven cognitive walkthroughs that put users' diverse problem-solving styles at the center stage of finding and fixing inclusivity issues.  
Historically, HCI practitioners leveraged GenderMag for a wide variety of user experience improvements such as inclusivity bug removal~\cite{Guizani22Inlcusivity}, task performance improvement~\cite{Vorvoreanu19Bias}, customer rating improvement~\cite{Burnett17MS}, etc. However, no prior GenderMag research has evaluated GenderMag's applicability and effectiveness within AI-powered systems. Addressing this gap in GenderMag studies, our goal is to investigate how successful GenderMag fixes can be in improving users' engagement and their mental models of AI.


